Stable Reinforcement Learning with Unbounded State Space

We consider the problem of reinforcement learning (RL) with unbounded state space motivated by the classical problem of scheduling in a queueing network. Traditional policies as well as error metric that are designed for finite, bounded or compact state space, require infinite samples for providing any meaningful performance guarantee (e.g. $\ell_\infty$ error) for unbounded state space. That is, we need a new notion of performance metric. As the main contribution of this work, inspired by the literature in queuing systems and control theory, we propose stability as the notion of "goodness": the state dynamics under the policy should remain in a bounded region with high probability. As a proof of concept, we propose an RL policy using Sparse-Sampling-based Monte Carlo Oracle and argue that it satisfies the stability property as long as the system dynamics under the optimal policy respects a Lyapunov function. The assumption of existence of a Lyapunov function is not restrictive as it is equivalent to the positive recurrence or stability property of any Markov chain, i.e., if there is any policy that can stabilize the system then it must possess a Lyapunov function. And, our policy does not utilize the knowledge of the specific Lyapunov function. To make our method sample efficient, we provide an improved, sample efficient Sparse-Sampling-based Monte Carlo Oracle with Lipschitz value function that may be of interest in its own right. Furthermore, we design an adaptive version of the algorithm, based on carefully constructed statistical tests, which finds the correct tuning parameter automatically.

==> appx_drift.tex <==
\section{Proof of Lemma~\ref{lem:hajek}} \label{sec:proof_drift}

\begin{proof}
Throughout the proof, we fix an $\eta\in(0, \min\{1, \alpha/(2c)\})$ and let $\rho = 1 - \eta\alpha/2$. To simplify the notation, we fix a $s_0$, and the probabilities and expectations should be understood as conditioned on $s_0 = s$ when appropriate.
Let $\mF_t$ denote the smallest 
$\sigma$-algebra containing all information pertaining to the MDP up to time $t$, i.e., $\{s_t\}_{t\geq 0}$ is adapted to $\{\mF_t\}_{t\geq0}$. 

We start by establishing Eq.~(\ref{eq:lem:hajek}). To do so, we will instead prove the following inequality, from which Eq.~(\ref{eq:lem:hajek}) can be readily obtained via Markov inequality:
\begin{equation}
    \E[e^{\eta L(s_t)}]\leq \rho^te^{\eta L(s_0)} + \frac{1-\rho^t}{1-\rho}e^{\nu + \eta B}.\label{eq:lem:hajek:proof1}
\end{equation}
Note that by Tower property, $\E[e^{\eta L(s_{t+1)}}] = \E[\E[e^{\eta L(s_{t+1})}|\mF_t]]$. Further,
\begin{equation}
    \E[e^{\eta L(s_{t+1})}|\mF_t] = \E[e^{\eta L(s_{t+1})}\mathbb{I}\{L(s_t)\leq B\}|\mF_t] + \E[e^{\eta L(s_{t+1})}\mathbb{I}\{L(s_t)> B\}|\mF_t]. \label{eq:lemma:hajek:proof2}
\end{equation}
We now analyze the two terms on the R.H.S. of the Eq.~(\ref{eq:lemma:hajek:proof2}) separately. For the first term,
\begin{align*}
    \E[e^{\eta L(s_{t+1})}\mathbb{I}\{L(s_t)\leq B\}|\mF_t] & = \E[e^{\eta (L(s_{t+1}) - L(s_{t}))}e^ {\eta L(s_t)}\mathbb{I}\{L(s_t)\leq B\}|\mF_t]\leq e^{\nu + \eta B},
\end{align*}
where the last inequality follows from the bounded increment condition and the fact that $\eta < 1$. For the second term of Eq.~(\ref{eq:lemma:hajek:proof2}),
\begin{align*}
    \E[e^{\eta L(s_{t+1})}\mathbb{I}\{L(s_t)> B\}|\mF_t] & = \E[e^{\eta (L(s_{t+1}) - L(s_{t}))}e^ {\eta L(s_t)}\mathbb{I}\{L(s_t)> B\}|\mF_t]\\
    &\leq \E[e^{\eta (L(s_{t+1}) - L(s_{t}))\mathbb{I}\{L(s_t)> B\}}|\mF_t] \cdot e^ {\eta L(s_t)}.
\end{align*}
We now show that $\E[e^{\eta (L(s_{t+1}) - L(s_{t}))\mathbb{I}\{L(s_t)> B\}}|\mF_t] \leq \rho$. Because of the bounded increment property, we know that $\E[e^{\eta (L(s_{t+1}) - L(s_{t}))\mathbb{I}\{L(s_t)> B\}}|\mF_t]$ has an absolutely convergent series expansion. That is,
\begin{align*}
  \E[e^{\eta (L(s_{t+1}) - L(s_{t}))\mathbb{I}\{L(s_t)> B\}}|\mF_t] &= 1 + \eta  \E[{(L(s_{t+1}) - L(s_{t}))\mathbb{I}\{L(s_t)> B\}}|\mF_t] \\
  & + \eta^2\sum_{k=2}^\infty\frac{\eta^{k-2}}{k!} \E[\big((L(s_{t+1}) - L(s_{t}))\mathbb{I}\{L(s_t)> B\}\big)^k|\mF_t]  \\
  & \leq 1 - \eta\alpha + \eta^2c.
\end{align*}
Note that since $\eta\in(0, \min\{1, \alpha/(2c)\})$, $1 - \eta\alpha + \eta^2c\leq 1- \eta\alpha/2 = \rho$. To summarize, we obtain that for Eq.~(\ref{eq:lemma:hajek:proof2}),
\begin{equation}
    \E[e^{\eta L(s_{t+1})}|\mF_t] \leq e^{\nu + \eta B} +  \rho e^{\eta L(s_t)}. \label{eq:lemma:hajek:proof3}
\end{equation}
By taking expectation on both side of Eq.~(\ref{eq:lemma:hajek:proof3}), we establish the following recursive equation:
\begin{equation*}
    \E[e^{\eta L(s_{t+1})}] \leq e^{\nu + \eta B} +  \rho \E[e^{\eta L(s_t)}].
\end{equation*}
Since Eq.~(\ref{eq:lem:hajek:proof1}) holds trivially for $t=0$, the above recursive equation implies that the desired inequality Eq.~(\ref{eq:lem:hajek:proof1}) is valid for all $t\ge 0$.

Next, we establish Eq.~(\ref{eq:lem:hajek:recurrent}) of Lemma \ref{lem:hajek}. Fix an $a\geq B$ and define $M(k) = \frac{e^{\eta L(s_k)}}{\rho^k}$. Recall that in the above proof, we showed that $\E[e^{\eta (L(s_{k+1}) - L(s_{k}))\mathbb{I}\{L(s_k)> B\}}|\mF_t] \leq \rho$. Therefore, $M(\min(k,T_a))$ is a non-negative supermartingale. This implies that $M(0)\geq \E[M(\min(k,T_a))]$, i.e.,
\begin{align*}
    e^{\eta L(s_0)}&\geq \E[e^{\eta Y_{\min(k,T_a)}}/ \rho^{\min(k, T_a)}]\\
    &\geq \E[e^{\eta Y_{\min(k,T_a)}}/ \rho^{\min(k, T_a)}\mathbb{I}\{T_a > k\}]\\
    &\geq \frac{e^{\eta a}}{\rho^k}\cdot \P(T_a > k),
\end{align*}
where the last inequality follows from the definition of $T_a$. This completes the proof of Eq.~(\ref{eq:lem:hajek:recurrent}).
\end{proof}



==> proof_proposition.tex <==
\begin{proof}[Proposition \ref{prop:delta_stability}]
To see why, recall the definition of level set, $\mathcal{C}(l)\triangleq \{s\in\mS\::\: L(s) \leq l \}$ and the assumption that the radius $r(\mathcal{C}(l))\triangleq$ $\sup_{s\in\mathcal{C}(l)}\Vert s\Vert_2 <\infty$ for every $l> 0 $. Now, Eq.~(\ref{eq:thm:stability}) implies that for some small $\epsilon>0$, we have
\begin{equation*}
    \lim\sup_{t\rightarrow\infty}\P\big(s_t\notin \mathcal{C}(b+\epsilon)|s_0=s\big)\leq \lim\sup_{t\rightarrow\infty}\P\big(L(s_t)\geq b|s_0=s\big)\leq \frac{1}{1-\rho}e^{\eta(B-b) +\nu}.
\end{equation*}
By letting $b\geq B$ and $b$ be large enough, we can always make the above probability bound as small as possible.
That is, given any small $\delta$, there exists large $b\geq B$ and a small $\epsilon$, such that
\begin{equation*}
    \lim_{t\rightarrow\infty}\P\big(s_t\notin \mathcal{C}(b+\epsilon)|s_0=s\big)\leq \delta,\quad\forall\:s\in\mS.
\end{equation*}
In addition, Eq.~(\ref{eq:thm:recurrent}) implies that 
\begin{equation*}
    \P\big(T_{b+\epsilon}(t) > k \:|\: s_t=s\big)\leq e^{{\eta}(L(s)- b-\epsilon)}\rho^k,\quad\forall\:s\in\mS\textrm{ and }\forall\:t\geq 0.
\end{equation*}
Therefore, 
\begin{equation*}
    \E\big[T_{b+\epsilon}(t)|s_t = s\big]=\sum_{k = 0}^\infty\P\big(T_{b+\epsilon}(t) > k|s_t = s\big)\leq e^{{\eta}(L(s)- b-\epsilon)}\cdot\frac{1}{1-\rho}<\infty.
\end{equation*}
That is, given the current state $s$, the return time to the bounded set $\mathcal{C}(b+\epsilon)$ is uniformly bounded, across all $t$. This completes the proof.
\end{proof}
